Non-invasive Inference of Thrombus Material Properties with Physics-informed Neural Networks

We employ physics-informed neural networks (PINNs) to infer properties of biological materials using synthetic data. In particular, we successfully apply PINNs on inferring the thrombus permeability and visco-elastic modulus from thrombus deformation data, which can be described by the fourth-order Cahn-Hilliard and Navier-Stokes Equations. In PINNs, the partial differential equations are encoded into the loss function, where partial derivatives can be obtained through automatic differentiation (AD). In addition, to tackling the challenge of calculating the fourth-order derivative in the Cahn-Hilliard equation with AD, we introduce an auxiliary network along with the main neural network to approximate the second-derivative of the energy potential term. Our model can predict simultaneously unknown parameters and velocity, pressure, and deformation gradient fields by merely training with partial information among all data, i.e., phase-field and pressure measurements, and is also highly flexible in sampling within the spatio-temporal domain for data acquisition. We validate our model by numerical solutions from the spectral/\textit{hp} element method (SEM) and demonstrate its robustness by training it with noisy measurements. Our results show that PINNs can accurately infer the material properties with noisy synthetic data, and thus they have great potential for inferring these properties from experimental multi-modality and multi-fidelity data.

==> sup.tex <==
% \subsubsection{Problem setup}
% Suppose we have a system of PDEs on $\Omega \subset \mathbb{R}^{n}, n = 1, 2, \textrm{or } 3$ :
% \begin{equation}
%     \mathcal{N}_{x}[\mathbf{u}(\mathbf{x}, t); \bm{\lambda}] = 0, (\mathbf{x}, t) \in \Omega \times [0, T], \bm{\lambda}\in \mathbb{R}^{m}, \label{equ: 14}
% \end{equation}
% with boundary and initial conditions:
% \begin{align}
%     \mathbf{u}(\mathbf{x}, t) &= \mathbf{u}_{0}(\mathbf{x}, t), t = t_{0}, \label{equ: 15}\\
%     \mathcal{B}_{x}[\mathbf{u}(\mathbf{x}, t)] &= g(\mathbf{x}, t), x \in \partial \Omega, \label{equ: 16}
% \end{align}
% $\mathcal{N}_{x}$ and $\mathcal{B}_{x}$ are a general differential operator and a boundary differential operator. Unlike the velocity field in the Cahn-Hilliard Navier-Stokes Equations, $\mathbf{u}(\mathbf{x}, t; \bm{\lambda})$ is the solution of the PDE system and $\lambda$ indicates the unknown PDE parameters. 

% Define a neural network:
% \begin{equation}
%     \mathbf{u}_{\mathcal{NN}} = \mathcal{NN}(\mathbf{x}^{*}, t^{*}; \bm{\theta}, \bm{\lambda}), (\mathbf{x}^{*}, t^{*}) \in \Omega \times [0, T], \bm{\lambda}\in \mathbb{R}^{m}, \bm{\theta} \in \Theta,
% \end{equation}
% where $\mathbf{u}_{\mathcal{NN}}$ is the output of the neural network, and $\theta \in \Theta$ is parameters (weights and biases) of the neural network. Given (part of) solution
% \begin{equation}
%     \mathbf{\hat{u}(\mathbf{x}^{*}, t^{*})}, (\mathbf{x}^{*}, t^{*}) \in \Omega \times [0, T], 
% \end{equation}
% within the same computational domian $\Omega$, the loss function of training process for a inverse PDE problem can be written as:
% \begin{align}
%     \argmin_{\theta^{*} \in \Theta, \bm{\lambda} \in \mathbb{R}^{m}}\mathcal{L}(\theta, \lambda)
% \end{align}
% where $\mathcal{L}$ is the linear combination of $\textit{L}_{2}$ residuals of equations \ref{equ: 14}, \ref{equ: 15}, \ref{equ: 16}, and the difference of model prediction $\mathbf{u}_{\mathcal{NN}} (\mathbf{x}^{*}, t^{*})$ and $\hat{\mathbf{u}(\mathbf{x}^{*}, t^{*})}$.
